Time Series Source Separation using Dynamic Mode Decomposition

The Dynamic Mode Decomposition (DMD) extracted dynamic modes are the non-orthogonal eigenvectors of the matrix that best approximates the one-step temporal evolution of the multivariate samples. In the context of dynamical system analysis, the extracted dynamic modes are a generalization of global stability modes. We apply DMD to a data matrix whose rows are linearly independent, additive mixtures of latent time series. We show that when the latent time series are uncorrelated at a lag of one time-step then, in the large sample limit, the recovered dynamic modes will approximate, up to a column-wise normalization, the columns of the mixing matrix. Thus, DMD is a time series blind source separation algorithm in disguise, but is different from closely related second order algorithms such as the Second-Order Blind Identification (SOBI) method and the Algorithm for Multiple Unknown Signals Extraction (AMUSE). All can unmix mixed stationary, ergodic Gaussian time series in a way that kurtosis-based Independent Components Analysis (ICA) fundamentally cannot. We use our insights on single lag DMD to develop a higher-lag extension, analyze the finite sample performance with and without randomly missing data, and identify settings where the higher lag variant can outperform the conventional single lag variant. We validate our results with numerical simulations, and highlight how DMD can be used in change point detection.

==> DMF Paper/Figures/AlgFlowChart.tex <==
\begin{tikzpicture}[node distance = 4cm, auto, thick, scale = 0.6, every node/.style = {transform shape}]
    % Place nodes
    \node [cloud] (init) {Data $X$};
    \node [decision, below of=init] (noisy) {Noisy or Missing Values?};
    \node [block, left=1cm of noisy] (noise) {Use rank $k$ truncated SVD (or OptShrink) to denoise data};
    \node [decision, below=1cm of noisy] (mean) {Mean $\bzr$?};
    \node [block, below left=1.6cm and 3cm of mean] (demean) {Estimate and subtract mean $\widehat{\mu}$ from data};
    \node [block, below=1cm  of mean] (dmd) {Perform DMD on (denoised, de-meaned) data};
    \node [circ, below=1cm  of dmd] (out) {Estimated modes $\widehat{Q}$, $\widehat{S}$, eigenvalues $\widehat{\lambda_i}$, mean $\widehat{\mu}$};

    % Draw edges
    \path [line] (init) -- (noisy);
    \path [line] (noisy) -- node [near start] {yes} (noise);
    \path [line] (noisy) -- node [near end] {no} (mean);
    \path [line] (noise) -- (mean);
    \path [line] (mean) -- node [near start] {no} (dmd);
    \path [line] (mean) -| node [near start] {yes} (demean);
    \path [line] (demean) -- (dmd);
    \path [line] (dmd) -- (out);
\end{tikzpicture}



==> DMF Paper/Figures/DMDFlowChart.tex <==
\begin{tikzpicture}[node distance = 4cm, auto, thick, scale = 0.6, every node/.style = {transform shape}]
    % Place nodes
    \node [cloud] (init) {Data $X$, Lag $\tau$, Rank $k$};
    \node [block, below=0.5cm of init] (A) {Form \\$\widehat{A} = X[:, (1 + \tau):n]$ \\$X[:, 1:(n - \tau)]^{+}$};
    \node [block, below=0.5cm of A] (eig) {Eigendecomposition of $\widehat{A}$: $\widehat{Q} \widehat{\Lambda} \widehat{Q}^{+}$};
    \node [block, below=0.5cm of eig] (sort) {Sort the eigenpairs by decreasing magnitude of $\widehat{\lambda}_i$};
    \node [block, below=0.5cm of sort] (trunc) {Truncate $\widehat{Q}$ to $\widehat{Q}[:, 1:k]$, $\widehat{\Lambda}$ to $\textrm{diag}(\widehat{\lambda}_1, \ldots, \widehat{\lambda}_k)$};
    \node [block, below=0.5cm of trunc] (S) {$\widehat{S}$ is $\widehat{C} = \left(\widehat{Q}[:, 1:k]^{+} X\right)^T$ with unit norm columns};
    \node [circ, below=0.5cm of S] (out) {Estimated modes $\widehat{Q}[:, 1:k]$, $\widehat{S}$, eigenvalues $\widehat{\lambda}_1, \ldots, \widehat{\lambda}_k$};

    % Draw edges
    \path [line] (init) -- (A);
    \path [line] (A) -- (eig);
    \path [line] (eig) -- (sort);
    \path [line] (sort) -- (trunc);
    \path [line] (trunc) -- (S);
    \path [line] (S) -- (out);
\end{tikzpicture}

==> Figures/AlgFlowChart.tex <==
\begin{tikzpicture}[node distance = 4cm, auto, thick, scale = 0.6, every node/.style = {transform shape}]
    % Place nodes
    \node [cloud] (init) {Data $X$};
    \node [decision, below of=init] (noisy) {Noisy or Missing Values?};
    \node [block, left=1cm of noisy] (noise) {Use rank $k$ truncated SVD (or OptShrink) to denoise data};
    \node [decision, below=1cm of noisy] (mean) {Mean $\bzr$?};
    \node [block, below left=1.6cm and 3cm of mean] (demean) {Estimate and subtract mean $\widehat{\mu}$ from data};
    \node [block, below=1cm  of mean] (dmd) {Perform DMD on (denoised, de-meaned) data};
    \node [circ, below=1cm  of dmd] (out) {Estimated modes $\widehat{Q}$, $\widehat{S}$, eigenvalues $\widehat{\lambda_i}$, mean $\widehat{\mu}$};

    % Draw edges
    \path [line] (init) -- (noisy);
    \path [line] (noisy) -- node [near start] {yes} (noise);
    \path [line] (noisy) -- node [near end] {no} (mean);
    \path [line] (noise) -- (mean);
    \path [line] (mean) -- node [near start] {no} (dmd);
    \path [line] (mean) -| node [near start] {yes} (demean);
    \path [line] (demean) -- (dmd);
    \path [line] (dmd) -- (out);
\end{tikzpicture}



==> Figures/DMDFlowChart.tex <==
\begin{tikzpicture}[node distance = 4cm, auto, thick, scale = 0.6, every node/.style = {transform shape}]
    % Place nodes
    \node [cloud] (init) {Data $X$, Lag $\tau$, Rank $k$};
    \node [block, below=0.5cm of init] (A) {Form \\$\widehat{A} = X[:, (1 + \tau):n]$ \\$X[:, 1:(n - \tau)]^{+}$};
    \node [block, below=0.5cm of A] (eig) {Eigendecomposition of $\widehat{A}$: $\widehat{Q} \widehat{\Lambda} \widehat{Q}^{+}$};
    \node [block, below=0.5cm of eig] (sort) {Sort the eigenpairs by decreasing magnitude of $\widehat{\lambda}_i$};
    \node [block, below=0.5cm of sort] (trunc) {Truncate $\widehat{Q}$ to $\widehat{Q}[:, 1:k]$, $\widehat{\Lambda}$ to $\textrm{diag}(\widehat{\lambda}_1, \ldots, \widehat{\lambda}_k)$};
    \node [block, below=0.5cm of trunc] (S) {$\widehat{S}$ is $\widehat{C} = \left(\widehat{Q}[:, 1:k]^{+} X\right)^T$ with unit norm columns};
    \node [circ, below=0.5cm of S] (out) {Estimated modes $\widehat{Q}[:, 1:k]$, $\widehat{S}$, eigenvalues $\widehat{\lambda}_1, \ldots, \widehat{\lambda}_k$};

    % Draw edges
    \path [line] (init) -- (A);
    \path [line] (A) -- (eig);
    \path [line] (eig) -- (sort);
    \path [line] (sort) -- (trunc);
    \path [line] (trunc) -- (S);
    \path [line] (S) -- (out);
\end{tikzpicture}
